$Q$-learning with Logarithmic Regret

This paper presents the first non-asymptotic result showing that a model-free algorithm can achieve a logarithmic cumulative regret for episodic tabular reinforcement learning if there exists a strictly positive sub-optimality gap in the optimal $Q$-function. We prove that the optimistic $Q$-learning studied in [Jin et al. 2018] enjoys a ${\mathcal{O}}\left(\frac{SA\cdot \mathrm{poly}\left(H\right)}{\Delta_{\min}}\log\left(SAT\right)\right)$ cumulative regret bound, where $S$ is the number of states, $A$ is the number of actions, $H$ is the planning horizon, $T$ is the total number of steps, and $\Delta_{\min}$ is the minimum sub-optimality gap. This bound matches the information theoretical lower bound in terms of $S,A,T$ up to a $\log\left(SA\right)$ factor. We further extend our analysis to the discounted setting and obtain a similar logarithmic cumulative regret bound.

==> broader.tex <==
%Our research broadens our understanding of model-free algorithms in RL, which in turn can help researchers design new principled algorithms and incorporate safety considerations for more complicated problems.
%This work does not present any foreseeable societal consequence.
We do not foresee any negative societal effects. We believe our algorithm can guide practitioners to design better algorithms that will potentially benefit the society. 

==> discounted.tex <==




==> proofs.tex <==
Before presenting the proof of Lemma~\ref{lemma:weighed-sum-learning-error}, we refer the readers to \cite{jin2018qlearning} for Lemma~\ref{lemma:property-lr} below, which summarizes the properties of $\alpha_t^i$ that will be useful in our proof.
\begin{lemma}[Properties of $\alpha_t^i$]
	\label{lemma:property-lr}
	Let $\alpha_t\!=\!\frac{H+1}{H+t}$, $\alpha_t^0\!=\!\prod_{j=1}^{t}\!\left(1\!-\!\alpha_{j}\right)$ and $\alpha_t^i\!=\!\alpha_i\!\prod_{j=i+1}^{t}\!\left(1\!-\!\alpha_{j}\right)$.
	\begin{enumerate}[(i)]
		\item $\sum_{i=1}^{t}\alpha_t^i=1$ and $\alpha_t^0=0$ for every $t\ge1$, $\sum_{i=1}^{t}\alpha_t^i=0$ and $\alpha_t^0=1$ for $t=0$.
		\item $\sum_{t=i}^{\infty}\alpha_t^i=1+\frac{1}{H}$ for every $i\ge1$. 
		%\item $\sqrt{\frac{\iota(t)}{t}}\le\sum_{i=1}^t\alpha_t^i\sqrt{\frac{\iota(i)}{i}}\le2\sqrt{\frac{\iota(t)}{t}}$.
	\end{enumerate}
\end{lemma}
%\begin{proof}[Proof of Lemma~\ref{lemma:weighed-sum-learning-error}]
%	We will recursively bound the weighted sum of step $h$ by its next step $(h\!+\!1)$, and unroll for $(H\!-\!h\!+\!1)$ steps for the desired bound. As suggested by Lemma~\ref{lemma: conc-event}, upper bounds of learning error holds under $\cE_{\mathrm{conc}}$. Thus we have
%		\begin{eqnarray}
%	&&\sum_{k=1}^K w_{k,h}
%	\left(Q_h^k-Q_h^*\right)\!\xahk{h}{k}\nonumber\\
%	&{\le}& \sum_{k=1}^K w_{k,h}\left(\alpha_{n_h^k}^0\! H\!+\!\sum_{i=1}^{n_h^k}\alpha_{n_h^k}^i\!\left(\!V_{\!h+1}^{\!\tau_h(s,a,i)}\!-\!V^*\!\right)\!\left(\!x_{h+1\!}^{\!\tau_h(s,a,i)}\!\right)\!+\!\beta_{\!n_h^k}
%	\right)\nonumber\\
%	&=& \sum_{k=1\atop n_h^k=0}^K w_{k,h} H+\sum_{k=1}^K w_{k,h} \beta_{n_h^k}
%	+\sum_{k=1}^K \left(V_{h+1}^k-V_{h+1}^*\right)\!\left(x_{h+1}^k\right)\!
%	\left(\!\sum_{i= n_h^k+1}^{N_h^K\!\xahk{h}{k}}\!
%	\alpha_{i}^{n_h^k}
%	w_{\tau_h(x_h^k,a_h^k,i),h}  \!\right)\nonumber\\
%	&\le& SAHw+\sum_{k=1}^K w_{k,h} \beta_{n_h^k}
%	+\sum_{k=1}^K w_{k,h\!+\!1}
%	\left(Q_{h+1}^k-Q_{h+1}^*\right)\!\xahk{h+1}{k}, \label{ineq:recursion}
%	\end{eqnarray}
%	The second term of Ineq~(\ref{ineq:recursion}) can be bounded from above in the following way:
%	\begin{align}
%	\sum_{k=1}^K w_{k,h} \beta_{n_h^k}&=
%	\sum_{s,a}\! \sum_{k=1\atop (s_h^k,a_h^k)=(s,a)}^{K}\!w_{k,h}\beta_{n_h^k}&\nonumber\\
%	&= 4c\sqrt{\!H^3\iota}
%	\sum_{s,a}\!
%	\sum_{i=1}^{N_h^{\!K}\!(s,a)}\!
%	\frac{w_{\!\tau\!(\!s,a,i\!),h}}{\sqrt{i}} & \left(\beta_t\!=\!4c\sqrt{\!\frac{H^3\iota}{t}}\right)\nonumber\\
%	&\le
%	4c\sqrt{\!H^3\iota}
%	\sum_{s,a}
%	\sum_{i=1}^{\left\lceil\frac{C^h_{s,a}}{w}\right\rceil}
%	\frac{w}{\sqrt{i}}&\left(\!\text{Rearrangement inequality, }
%	C_{\!s,a\!}^h\!:=\!\sum\nolimits_{i=1}^{n_h^{\!K}\!(\!s,a\!)}\!w_{\!\tau\!(\!s,a,i\!),h}\!\right)
%	\nonumber\\
%	&\le10c\sqrt{H^3\iota}
%	\sum_{s,a}\sqrt{C_{s,a}^h w}&(\text{Integral conversion})\nonumber\\
%	&\le10c\sqrt{SACwH^3\iota}.
%	&\left(\text{Cauchy inequality, }
%	\sum\nolimits_{\!s,a\!}\!C_{\!s,a\!}^h\!=\!\sum\nolimits_{k=1}^K w_k\!\le\!C\right)
%	\label{ineq:beta-sum}
%	\end{align}
%	
%	For the third term in Ineq (\ref{ineq:recursion}), we notice that $\Vxhk{h+1}{k}=\Qxahk{h+1}{k}$ due to greedy choice of actions and $V_{h+1}^*\!(x_{h+1}^k)\ge Q_{h+1}^*\!(x_{h+1}^k)$ by definition. For the weights we
%	let $$w_{k,h\!+\!1}=
%	\sum_{i= n_h^k+1}^{N_{\!h}^{\!K}\!\xahk{h}{k}}\!
%	w_{\tau_h\!\left(\!x_h^k,a_h^k,i\!\right)\!,h} \alpha_{i}^{\!n_h^k}.$$
%	 It then follows directly from Lemma~\ref{lemma:property-lr} that $\left\{w_{k,h\!+\!1}\right\}_{k\in[K]}$ is a $\left(C,\left(\!1\!+\!\frac{1}{H}\!\right)\!w\right)$-sequence, as derived below.
%	\begin{eqnarray}
%	w_{k\!,h\!+\!1}\le w\! \sum_{i\ge n_h^k} \!\alpha_i^{n_h^k}
%	\le  \left(\!1\!+\!\frac1H\!\right)\!w,\qquad
%	\sum_{k=1}^{K}w_{k,h\!+\!1}%=\sum_{k=1}^{K}\sum_{i= n_h^k+1}^{N_h^K\!\xahk{h}{k}}\!
%	%\!w_{\tau_h\!\left(x_h^k,a_h^k,i\right),h} \alpha_{i}^{n_h^k}
%	=\sum_{i=1}^K w_{i,h}\sum_{t\le n_h^i}\!\alpha_{n_h^i}^{k}
%	=\sum_{i=1}^K w_{i,h}\le C. \label{ineq:w_{h+1}}
%	\end{eqnarray}
%	 Plugging Ineq (\ref{ineq:beta-sum}) and (\ref{ineq:w_{h+1}}) back to Ineq (\ref{ineq:recursion}) gives
%	 \begin{eqnarray}
%	 \sum_{k=1}^K \!w_{k,h}\!
%	 \left(\!Q_h^k\!-\!Q_h^*\!\right)\!\xahk{h}{k}
%	 \!\le\! SAHw\!+\!10c\sqrt{SACwH^3\iota}
%	 \!+\!\sum_{k=1}^K\!w_{k,h\!+\!1}\!
%	 \left(\!Q_{h\!+\!1}^k\!-\!Q_{h\!+\!1}^*\!\right)\!\xahk{h+1}{k},
%	 \end{eqnarray}
%	 where the third term is a weighted sum of learning errors in level $h+1$, with weights $\left\{\!w_{k,\!h\!+\!1\!}\right\}_{\!k\in[\!K\!]\!}$ being $\left(\!C,\left(\!1\!+\!{1}\!/\!{H}\!\right)\!w\!\right)$-sequence.
%	 Recursing this argument for $h\!+\!1,h\!+\!2,\!\cdots\!,\!H$ yields
%	 \begin{eqnarray}
%	 \sum_{k=1}^K \!w_{k,h}\!
%	 \left(\!Q_h^k\!-\!Q_h^*\!\right)\!\xahk{h}{k}
%	 &\le&\sum_{h'=0}^{H-h}\left(SAH\left(\!1\!+\!{1}\!/\!{H}\!\right)^{h'}w\!+\!10c\sqrt{SAC\left(\!1\!+\!{1}\!/\!{H}\!\right)^{h'}wH^3\iota}\right)\nonumber\\
%	 &\le&H\left(SAHew\!+\!10c\!\sqrt{SACewH^3\iota}\right).
%	 \end{eqnarray}
%	 which is the desired conclusion.
%\end{proof}
%

